Checking Presence Reachability Properties on Parameterized Shared-Memory Systems

We consider the verification of distributed systems composed of an arbitrary number of asynchronous processes. Processes are identical finite-state machines that communicate by reading from and writing to a shared memory. Beyond the standard model with finitely many registers, we tackle round-based shared-memory systems with fresh registers at each round. In the latter model, both the number of processes and the number of registers are unbounded, making verification particularly challenging. The properties studied are generic presence reachability objectives, which subsume classical questions such as safety or synchronization by expressing the presence or absence of processes in some states. In the more general round-based setting, we establish that the parameterized verification of presence reachability properties is PSPACE-complete. Moreover, for the roundless model with finitely many registers, we prove that the complexity drops down to NP-complete and we provide several natural restrictions that make the problem solvable in polynomial time.

==> notions.tex <==
\knowledge{notion}
| register protocols@rl
| roundless register protocol
| roundless register protocols
| Roundless register protocols
| protocol@rl

\knowledge{notion}
| register protocols@rb
| round-based register protocol
| round-based register protocols
| Round-based register protocols
| protocol@rb


\knowledge{notion}
| size@roundless

\knowledge{notion}
| concrete configuration@rl
|concrete@rl

\knwoledge{notion}
| abstract configuration@rl
| abstract@rl

\knowledge{notion}
| concrete configuration@rb
|concrete@rb

\knwoledge{notion}
| abstract configuration@rb
| abstract@rb

\knowledge{notion}
| initial@rl

\knowledge{notion}
| successor@concrete

\knowledge{notion}
|successor@abstract

\knowledge{notion}
| step

\knowledge{notion}
| destination

\knowledge{notion}
| execution@concrete
| concrete execution

\knowledge{notion}
| execution@abstract
| abstract execution

\knowledge{notion}
| reachable@concrete
| reachability@concrete

\knowledge{notion}
| reachable@abstract
| reachability@abstract

\knowledge{notion}
| coverability problem@rl
| cover@rl

\knowledge{notion}
| cover@rb

\knowledge{notion}
| target problem@rl
| target@rl

\knowledge{notion}
| target@rb

\knowledge{notion}
| presence constraint@rl
| presence constraints@rl
| Presence constraint@rl
| Presence constraints@rl

\knowledge{notion}
| presence constraint@rb
| presence constraints@rb
| Presence constraint@rb
| Presence constraints@rb
| round-based presence constraint

\knowledge{notion}
| atomic proposition@rl
|atomic propositions@rl


\knowledge{notion}
| atomic proposition@rb
| atomic propositions@rb

\knowledge{notion}
| Presence Reachability Problem@rl
| PRP@rl

\knowledge{notion}
| Presence Reachability Problem@rb
| PRP@rb
| round-based presence reachability problem
| round-based \PRP 
| Round-based \PRP 


\knowledge{notion}
| DNF Presence Reachability Problem@rl
| \dnfPRP@rl

\knowledge{notion}
| Presence Reachability Problem@rb
| \PRP@rb

\knowledge{notion}
| projection@abstraction

\knowledge{notion}
| reachability set@concrete
|\creach

\knowledge{notion}
 | reachability set@abstract
| \areach 

\knowledge{notion}
| uninitialized
| Uninitialized

\knowledge{notion}
| saturation

\knowledge{notion}
| synchronizing execution

\knowledge{notion}
| location
| locations

\knowledge{notion}
| move 
| moves 

\knowledge{notion}
| effect

\knowledge{notion}
| on round 

\knowledge{notion}
| desertion
| desert
| deserts
| deserting
| non-deserting

\knowledge{notion}
| footprint
| footprints

\knowledge{notion}
| local configuration
| local configurations

\knowledge{notion}
| projection@fp

\knowledge{notion}
|visibility range 
| \vrange

\knowledge{notion}
| normal form@rl 

\knowledge{notion}
| normal form@rb

\knowledge{notion}
| \populated




